On Scheduler Side-Channels in Dynamic-Priority Real-Time Systems

While the existence of scheduler side-channels has been demonstrated recently for fixed-priority real-time systems (RTS), there have been no similar explorations for dynamic-priority systems. The dynamic nature of such scheduling algorithms, e.g., EDF, poses a significant challenge in this regard. In this paper we demonstrate that side-channels exist in dynamic priority real-time systems. Using this side-channel, our proposed DyPS algorithm is able to effectively infer, with high precision, critical task information from the vantage point of an unprivileged (user space) task. Apart from demonstrating the effectiveness of DyPS, we also explore the various factors that impact such attack algorithms using a large number of synthetic task sets. We also compare against the state-of-the-art and demonstrate that our proposed DyPS algorithms outperform the ScheduLeak algorithms in attacking the EDF RTS.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Sections/reconstruct_observer_phase.tex <==
\section{Reconstructing The Observer Task's Phase}

In Section~\ref{sec:observing_victim_arrivals}

%================================%
%========== Subsection ==========%
%================================%
\subsection{Reconstruction with Start Times}
\label{sec:infer_phi_o}
Reconstructing the observer task's phase $\phi_o$ is carried out on the observer task itself.
When a new job of the observer task gets to run, $a_o$ is unknown since there might be higher priority tasks delaying the observer task's execution. However, what the observer task itself can learn is the job's start time $s_i$ which is bounded by $a_o \leq s_o \leq d_o-C_o$.
Let $\widetilde{\phi_o}$ be the task phase inferred by the observer task.
%Ideally, if we know that there exists a job whose $s_o$ is equal to $a_o$, then w
For a given job, we may compute the inference of the task phase by
\begin{equation}
\label{eq:infer_phio}
    \widetilde{\phi_o} = s_o \mmod T_o
\end{equation}
where $T_o$ is known to the attacker. %This yields $\widetilde{\phi_o}=\phi_o$ where $\phi_o = a_o \mod T_o$.
Intuitively, the closer $s_o$ is to $a_o$, the better the inference $\widetilde{\phi_o}$ will be.
With collecting and examining more start times, the attacker may further improve the inference of the task phase by determining the closest $s_o$ to $a_o$ and then computing $\widetilde{\phi_o}$ using Equation~\ref{eq:infer_phio}. 
When there exists one job whose $s_o$ is equal to $a_o$, the correct task phase can be inferred $\widetilde{\phi_o}=\phi_o$.
In \hl{Section~XXX} we discuss the factors that impact the inference and how likely the attacker experiences $s_o=a_o$ in a given task set.
What follows formally describes the algorithms.

Consider the observer task launching the attack at $k$-th job ($k$ is an arbitrary number that is unknown to the attacker) and collect its own job start times for $m$ jobs. What the observer task gets is a set of start times of consecutive jobs $S^{observed}_o=\{s^k_o, s^{k+1}_o,...,s^{k+m-1}_o\}$.
Our goal is to find the start time that is closest to its arrival time.
We do this by comparing the start times with using the following proposition:

\begin{proposition}
\label{prop:closer_s}
Given two start times $s^k_o$ and $s^{k+p}_o$ where $p \geq 1$, we can determine the start time that is closer to its arrival time to be
\begin{equation}
    \begin{cases}
    s^k_o & \text{if } s^k_o < s^{k+p}_o-p \cdot T_o\\
    s^{k+p}_o & \text{otherwise.}
\end{cases}
\end{equation}
\end{proposition}
\begin{proof}
\hl{(Proof may be simplified.)}
The given start time pair represents two jobs differing in $p$ periods.
Therefore, the start time of the $(k+p)$-th job can be shifted to the period the same as the $k$-th job by $s^{k+p}_o-j \cdot T_o$ since the observer task arrives periodically (\ie $a^k_o=a^{k+p}_o-j \cdot T_o$).
As a result, the two start times on the same period ($s^k_o$ and the shifted $s^{k+p}_o-p \cdot T_o$) are comparable.
The smaller one is closer to its arrival time since $a_o \leq s_o$.
\end{proof}

By employing Proposition~\ref{prop:closer_s}, the start time closest to its arrival time can be determined from $S^{observed}_o$ and the inference of the task phase of the observer task can be computed by
\begin{equation}
\label{eq:infer_phi_o_full}
    \widetilde{\phi_o}=\min(s_o^{k+p}-p \cdot T_o \mid 0 \leq p < m) \mmod T_o
\end{equation}
where $T_o$ is the period known to the attacker and $k$ can be unknown.
Then, given a start time $s_o$, the attacker can compute its projected arrival time $\widetilde{a_o}$ by
\begin{equation}
\label{eq:inferred_a_o}
    \widetilde{a_o}=s_o-\widetilde{j_o}
    %\widetilde{a_o}=s_o-[(s_o \mod T_o)-\widetilde{\phi_o}]\mod T_o
\end{equation}
where 
%$\widetilde{j_o}=[(s_o \mmod T_o)-\widetilde{\phi_o}] \mmod T_o$ 
$\widetilde{j_o}=(s_o-\widetilde{\phi_o}) \mmod T_o$ 
represents the delay such a job may have experienced.

\begin{example}
\label{ex:infer_phi_o}
Let's consider the task set given in Example~\ref{ex:infer_phi_v}.
Assume that the observer task starts collecting its start times for $10$ instances since the job starting at $t=41$.
The collected start times are $S^{observed}_o=\{41,53,61,71,81,92,101,111,121,133\}$. By using Equation~\ref{eq:infer_phi_o_full}, the inference of the observer task's phase can be computed by 
$\widetilde{\phi_o}=\min(41,43,41,41,41,42,41,41,41,43) \mmod 10=1$.
%Let's assume that the attacker starts collecting the observer task's start times for $10$ periods since the system begins at the time point $t=0$.
%The collected start times are $S^{observed}_o=\{1,13,21,31,41,53,61,71,81,92\}$. By using Equation~\ref{eq:infer_phi_o_full}, the inference of the observer task's phase can be computed by 
%$\widetilde{\phi_o}=\min(1,3,1,1,1,3,1,1,1,2) \mmod 10=1$.
In this example, $\widetilde{\phi_o}=\phi_o=1$ and thus the correct observer task's phase is obtained.
\qedsymbol
\end{example}


%================================%
%========== Subsection ==========%
%================================%
\subsection{Analysis}
In last section we present algorithms that can reconstruct the observer task's phase by using the start times of its own jobs.
When there exists at least one job of the observer task whose arrival time equals its start time (\ie the job is not delayed by any higher priority task and thus $a_o=s_o$), the correct task phase can be reconstructed.
In contrast, the correct inference cannot be made if the starts of the observer task consistently suffer some delays in every period. 
%Yet, this would mean that there exist some execution intervals that constantly appear at the observer task's arrival time points and have priorities higher than the observer task. 
In this section we study the factors that may contribute to the delays in the observer task's start times.
%Proposition~\ref{prop:ToObserveTv} shows that a task's arrival can only be observable by a task with larger period. It also means that a task's start times can only be delayed by the tasks that have smaller periods. Therefore, we only need to focus on the interference coming from the tasks with smaller periods here.
We start off by considering the interference from one task.
\hl{(CY's Note: removed the condition that says only $\tau_i$, $T_i<T_o$, can influence the arrivals of $\tau_o$.)}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\columnwidth]{Figures/ex_equal_arrival_offset.pdf}
    \caption{An example of the projection of the observer task's arrivals on a task's period for Proposition~\ref{prop:a_o_interfered_by_one_task}. In this example an observer task $\tau_o$ ($T_o=10$) and a periodic task $\tau_1$ ($T_1=8$) are considered. It shows that the projected arrivals of $\tau_o$ appear every $\sigma(T_o,T_1)T_1=2$ time columns.}
    \label{fig:ex_equal_arrival_offset}
\end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.99\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{Figures/ex_interfered_by_one_harmonic_task.pdf}
        %\vspace{-1\baselineskip}
        \caption{When $\phi_1=0$ and $\phi_o=1$, all the arrivals of $\tau_o$ are interfered by the harmonic task $\tau_1$.}
    \end{subfigure}%  
    %\hfill  
    \vspace{1\baselineskip}
    \begin{subfigure}[t]{0.99\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{Figures/ex_not_interfered_by_one_harmonic_task.pdf}
        %\vspace{-1.3\baselineskip}
        \caption{When $\phi_1=0$ and $\phi_o=2$, no arrival of $\tau_o$ is interfered by the harmonic task $\tau_1$.}
	%\label{fig:arrv_seg_b}
    \end{subfigure}
    %\vspace{-0.3\baselineskip}
    \caption{Schedules of the task set $\Gamma=\{\tau_o, \tau_1\}$ given in Example~\ref{ex:psi_with_harmonic_task}. The $T_o$ and $T_i$ are in harmony and thus $\psi(\tau_o,\tau_1)=1$.}
    \label{fig:ex_interference_of_one_harmonic_task}
    %\vspace{-0.5\baselineskip}
\end{figure*}

\begin{proposition}
\label{prop:a_o_interfered_by_one_task}
Given an observer task $\tau_o$ and a periodic task $\tau_i$, %with a smaller period (\ie $T_i<T_o$), 
the maximum proportion of the arrivals of $\tau_o$ may be interfered solely by the task $\tau_i$ is computed by 
\begin{equation}
\label{eq:psi_of_taski}
    \psi(\tau_o,\tau_i)= \left\lceil \frac{u_i}{\sigma_{(\tau_o,\tau_i)}} \right\rceil \sigma_{(\tau_o,\tau_i)}
\end{equation}
where $u_i=\frac{C_i}{T_i}$ is the utilization of $\tau_i$, $\sigma_{(\tau_o,\tau_i)}=\frac{T_o}{LCM(T_o,T_i)}$ is the inverse of the number of the arrivals of $\tau_o$ in a $LCM(T_o,T_i)$ and the resulting $\psi(\tau_o,\tau_i)$ is a fraction with a range  $0 < \psi(\tau_o,\tau_i) \leq 1$.
\end{proposition}
\begin{proof}
Since both tasks are periodic, the schedule of the two tasks repeats after their \textit{least common multiple}, $LCM(T_o, T_i)$. There are $\frac{LCM(T_o,T_i)}{T_o}$ arrivals of $\tau_o$ in a $LCM(T_o, T_i)$. By projecting these arrivals of $\tau_o$ onto a timeline with length equal to the period of $\tau_i$, an arrival of $\tau_o$ appears every $\frac{1}{\frac{LCM(T_o,T_i)}{T_o}} \cdot T_i = \sigma_{(\tau_o,\tau_i)} T_i$ time units and repeats after each $LCM(T_o, T_i)$ \cite[Observation 2]{chen2019novel}, as illustrated in Figure~\ref{fig:ex_equal_arrival_offset}.
The most number of arrivals of $\tau_o$ may be interfered by the execution of $\tau_i$ in one $LCM(T_o, T_i)$ is computed by $\left \lceil \frac{C_i}{\sigma_{(\tau_o,\tau_i)} T_i} \right \rceil = \left \lceil \frac{u_i}{\sigma_{(\tau_o,\tau_i)}} \right \rceil$ which happens when there exists an instant at which both tasks arrive at the same time (\eg when $\phi_o = \phi_i$). 
Then, the maximum proportion of the arrivals of $\tau_o$ may be interfered by $\tau_i$ in one $LCM(T_o, T_i)$ can be computed by 
$\psi(\tau_o,\tau_i) = \left\lceil \frac{u_i}{\sigma_{(\tau_o,\tau_i)}} \right\rceil \sigma_{(\tau_o,\tau_i)}$.
Since this relation is the same across all $LCM(T_o, T_i)$, the calculated $\psi(\tau_o,\tau_i)$ applies to the whole schedule. 
\end{proof}

When $\psi(\tau_o,\tau_i)<1$, it means that at least $1-\psi(\tau_o,\tau_i)$ of the arrivals of $\tau_o$ are not interfered by $\tau_i$. % (and thus $a_o=s_o$ for those intact instances).
In contrast, when $\psi(\tau_o,\tau_i)=1$, it is possible for the execution of $\tau_i$ to interfere all the arrivals of $\tau_o$, which would result in an inaccurate $\widetilde{\phi_o}$.
Intuitively, it can happen when $\tau_i$ has a period in harmony with that of $\tau_o$.  An example is given as follows.

\hl{Hint: We seek where it fails from the simplest case: with 2 tasks.}
\begin{example}
\label{ex:psi_with_harmonic_task}
Consider an observer task $\tau_o$ ($T_o=10$, $C_o=4$) and a task $\tau_1$ ($T_1=5$, $C_1=2$). The two tasks are in harmony because $T_o \mmod T_1=0$. Then $\psi(\tau_o,\tau_1)$ is computed by
%
\begin{equation*}
\sigma_{(\tau_o,\tau_1)}=\frac{T_o}{LCM(T_o,T_1)}=1
\end{equation*}
\begin{equation*}
\psi(\tau_o,\tau_1)= \left\lceil \frac{u_1}{\sigma_{(\tau_o,\tau_1)}} \right\rceil \sigma_{(\tau_o,\tau_1)}=\left\lceil u_1 \right\rceil=1
\end{equation*}
%
which indicates that all the arrivals of $\tau_o$ may be interfered by $\tau_1$. 
Figure~\ref{fig:ex_interference_of_one_harmonic_task} illustrates two possible schedules for the given task set. Figure~\ref{fig:ex_interference_of_one_harmonic_task}(a) shows the case where $\phi_o=1$ and $\phi_1=0$, all the arrivals of $\tau_o$ are interfered by $\tau_1$.
Figure~\ref{fig:ex_interference_of_one_harmonic_task}(b) shows the case where $\phi_o=2$ and $\phi_1=0$, all the arrivals of $\tau_o$ are no longer interfered by $\tau_1$.
\qedsymbol

\end{example}

The above example shows a crucial fact that $\psi(\tau_o,\tau_i)$ only represents the upper bound of the interference (when only such a task is considered). That is, having $\psi(\tau_o,\tau_i)=1$ does not mean all the arrivals of $\tau_o$ are absolutely interfered. 
With the same task set but different task phases (which can vary across systems and every time the system restarts), the impact of the interference can be quite different, as shown in Example~\ref{fig:ex_interference_of_one_harmonic_task}.

On the other hand, the schedules presented in Figure~\ref{fig:ex_interference_of_one_harmonic_task} are generated based on WCETs. However, the actual run-time execution times in real systems can vary throughout the time. As a result, the run-time task utilization is in fact smaller and, based on Equation~\ref{eq:psi_of_taski}, the proportion of arrivals of the observer task is also smaller. 
Taking the schedule in Figure~\ref{fig:ex_interference_of_one_harmonic_task}(a) as an example, if the first instance's execution time of $\tau_1$ is $c_1^1=1$ (rather than its WCET), then the arrival $a_o^1$ of the observer task will not be interfered. In such a case, $s_o^1=a_o^1$ and the correct task phase inference becomes possible.
Therefore, the actual impact is highly dependent on the task phases as well as the run-time variations.

We now turn our focus to the interference caused by multiple tasks (again, with periods smaller than $T_o$).
We have the following Proposition to evaluate the interference:

\hl{Hint: It is useful if we can at least prove that it is an upper-bound. Otherwise we don't even show this proposition.}
\hl{TODO: We'll have to see if we want to restrict the following to $\tau_i\in\Gamma-\{\tau_o\} \& T_i<T_o$}
\begin{proposition}
Given a task set $\Gamma$ and an observer task $\tau_o\in\Gamma$, the maximum proportion of the arrivals of $\tau_o$ may be interfered by all other tasks in the task set is computed by
\begin{equation}
    \varUpsilon(\Gamma, \tau_o)=\min(1.0, \hspace{-1em} \sum_{\tau_i\in\Gamma-\{\tau_o\}} \hspace{-1em} \psi(\tau_o,\tau_i))
\end{equation}
where $\psi(\tau_o,\tau_i)$ is computed by Equation~\ref{eq:psi_of_taski} and the resulting $\varUpsilon(\Gamma, \tau_o)$ is a fraction with a range  $0 < \varUpsilon(\Gamma, \tau_o) \leq 1$.

\end{proposition}
\begin{proof}
\todo[inline]{What follows is for internal discussion.}
\hl{Question: How should interference from two or more tasks be combined and how to prove it?}
\hl{Ideas: When combining interference from two or more tasks, two things should be considered:
(a) when multiple tasks are scheduled together, execution intervals are added up making a longer execution intervals, which potentially could interfere the arrival(s) that is not interfered when interference from each task is examined individually. So more arrivals may be interfered from this aspect. (b) on the other hand, multiple tasks may contribute to interfering the same arrival when each task is examined individually. When combined, that arrival is only counted once, so the actual number of arrivals being interfered is lower from this aspect.
}
%v - v - v - v - v - v - 1/2
%v - - v - - v - - v - - 1/3
%- - - - - v - - - - - v 1/6
\end{proof}
